Tweetorial Hooks: Generative AI Tools to Motivate Science on Social Media

Communicating science and technology is essential for the public to understand and engage in a rapidly changing world. Tweetorials are an emerging phenomenon where experts explain STEM topics on social media in creative and engaging ways. However, STEM experts struggle to write an engaging "hook" in the first tweet that captures the reader's attention. We propose methods to use large language models (LLMs) to help users scaffold their process of writing a relatable hook for complex scientific topics. We demonstrate that LLMs can help writers find everyday experiences that are relatable and interesting to the public, avoid jargon, and spark curiosity. Our evaluation shows that the system reduces cognitive load and helps people write better hooks. Lastly, we discuss the importance of interactivity with LLMs to preserve the correctness, effectiveness, and authenticity of the writing.

==> figures/a_deactivated_table_study1pvalue.tex <==

% {\setstretch{0.9}
\begin{table}[!h]
\centering
\begin{tabular}{|l|l|l|l|} 
\hline
& PS1 & PS2 & PS3  \\ 
\hline
R1: Jargon-Free     & \makecell{3.92\\p=.997}& \makecell{3.82\\p=.979}  & \makecell{3.62\\\newline}   \\ 
\hline
R2: Examples & \makecell{2.28\\\textbf{p<.001}}   & \makecell{3.24\\p=.081}  & \makecell{3.40\\\newline}   \\ 
\hline
R3: Sparks Curiosity     & \makecell{2.58\\\textbf{p<.001}}  & \makecell{3.40\\p=.461}  & \makecell{3.40\\\newline}  \\ 
\hline

Overall & \makecell{2.93\\\textbf{p<.001}}  & \makecell{3.49\\p=.694}  & \makecell{3.47\\\newline}   \\
\hline

\end{tabular}
\label{tab:annotation_statistics}
\caption{Average scores for each prompting strategy based on rubric performances and their p-values for the paired-sample Wilcoxon tests with PS3. Bolded p-values are statistically significant, showing that the R2, R3, and overall scores of PS3 are significantly higher than those of PS1.}
\end{table}
% }

==> figures/a_deactivated_table_study2pvalue.tex <==

\begin{table*}[!h]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|} 
\hline
 Condition & 
  Mental Demand & 
 Effort &
 Frustration &
Performance & 
 Physical Demand &
 Temporal Demand	
  \\ 
\hline
With the system &	
2.87 &	
2.87 &	
1.93  &
5.73 &	
1.10 &
2.37
\\
\hline
Without the system &	
4.00 & 
4.40&	
2.77 &
4.50&
1.37 &	
2.40
 \\ 
\hline

p-value &	
\textbf{0.004} &	
\textbf{0.002}  & 
\textbf{0.02} &
\textbf{0.001} &
0.08 & 
0.598	
\\


\hline
\end{tabular}
\caption{User study TLX results and p-values for the Wilcoxon tests
are reported. Bolded p-values are statistically significant.}
\label{tab:userstudy_statistics}
\end{table*}

